Quantum Multi-Agent Reinforcement Learning for Autonomous Mobility Cooperation

For Industry 4.0 Revolution, cooperative autonomous mobility systems are widely used based on multi-agent reinforcement learning (MARL). However, the MARL-based algorithms suffer from huge parameter utilization and convergence difficulties with many agents. To tackle these problems, a quantum MARL (QMARL) algorithm based on the concept of actor-critic network is proposed, which is beneficial in terms of scalability, to deal with the limitations in the noisy intermediate-scale quantum (NISQ) era. Additionally, our QMARL is also beneficial in terms of efficient parameter utilization and fast convergence due to quantum supremacy. Note that the reward in our QMARL is defined as task precision over computation time in multiple agents, thus, multi-agent cooperation can be realized. For further improvement, an additional technique for scalability is proposed, which is called projection value measure (PVM). Based on PVM, our proposed QMARL can achieve the highest reward, by reducing the action dimension into a logarithmic-scale. Finally, we can conclude that our proposed QMARL with PVM outperforms the other algorithms in terms of efficient parameter utilization, fast convergence, and scalability.

==> bio.tex <==


\begin{IEEEbiographynophoto}{Dr. Soohyun Park} is a postdoctoral scholar at Korea University, Seoul, Republic of Korea, since 2023, where she received her Ph.D. in electrical and computer engineering. Her research focuses include deep learning algorithms and their applications. She was a recipient of the IEEE Vehicular Technology Society (VTS) Seoul Chapter Award in 2019.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Jae Pyoung Kim} is currently an M.S. student in electrical and computer engineering at Korea University, Seoul, Republic of Korea, since March 2023. 
His current research interests include quantum machine learning. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Chanyoung Park} is currently a Ph.D. student in Electrical and Computer Engineering at Korea University, Seoul, Republic of Korea, since September 2022. His research focuses include deep learning algorithms and their applications to networks. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Prof. Soyi Jung} has been an assistant professor at Ajou University, Suwon, Republic of Korea, since September 2022. Before joining Ajou University, she was an assistant professor at Hallym University, Chuncheon, Republic of Korea, from 2021 to 2022; a visiting scholar at Donald Bren School of Information and Computer Sciences, University of California, Irvine, CA, USA, from 2021 to 2022. She received her B.S., M.S., and Ph.D. degrees in electrical and computer engineering from Ajou University, Suwon, Republic of Korea, in 2013, 2015, and 2021, respectively. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}
{Prof. Joongheon Kim} (M'06--SM'18) has been with Korea University, Seoul, Korea, since 2019, where he is currently an associate professor. He received the Ph.D. degree in computer science from the University of Southern California (USC), Los Angeles, CA, USA, in 2014. Before joining Korea University, he was a systems engineer with Intel Corporation (Santa Clara, CA, USA, 2013--2016) and an assistant professor with Chung-Ang University (Seoul, Korea, 2016--2019). 
He serves as an editor for \textsc{IEEE Transactions on Vehicular Technology}, \textsc{IEEE Transactions on Machine Learning in Communications and Networking}, and \textsc{IEEE Communications Standards Magazine}. 
He was a recipient of USC Annenberg Graduate Fellowship with his Ph.D. admission (2009), Intel Corporation Next Generation and Standards Division Recognition Award (2015), \textsc{IEEE Systems Journal} Best Paper Award (2020), IEEE ComSoc Multimedia Communications Technical Committee (MMTC) Outstanding Young Researcher Award (2020), and IEEE ComSoc MMTC Best Journal Paper Award (2021). 
\end{IEEEbiographynophoto}

